Follow the Scent: Defeating IPv6 Prefix Rotation Privacy

IPv6's large address space allows ample freedom for choosing and assigning addresses. To improve client privacy and resist IP-based tracking, standardized techniques leverage this large address space, including privacy extensions and provider prefix rotation. Ephemeral and dynamic IPv6 addresses confound not only tracking and traffic correlation attempts, but also traditional network measurements, logging, and defense mechanisms. We show that the intended anti-tracking capability of these widely deployed mechanisms is unwittingly subverted by edge routers using legacy IPv6 addressing schemes that embed unique identifiers. We develop measurement techniques that exploit these legacy devices to make tracking such moving IPv6 clients feasible by combining intelligent search space reduction with modern high-speed active probing. Via an Internet-wide measurement campaign, we discover more than 9M affected edge routers and approximately 13k /48 prefixes employing prefix rotation in hundreds of ASes worldwide. We mount a six-week campaign to characterize the size and dynamics of these deployed IPv6 rotation pools, and demonstrate via a case study the ability to remotely track client address movements over time. We responsibly disclosed our findings to equipment manufacturers, at least one of which subsequently changed their default addressing logic.

==> bibliography.tex <==
\begin{thebibliography}{10}

\bibitem{ieee802}
{IEEE Standard for Local and Metropolitan Area Networks: Overview and
  Architecture}.
\newblock {\em {IEEE Std 802-2014 (Revision to IEEE Std 802-2001)}}, pages
  1--74, 2014.

\bibitem{avm}
{AVM}, 2020.
\newblock \url{https://en.avm.de/}.

\bibitem{bihnet}
{BH Telecom}, 2020.
\newblock \url{https://www.bhtelecom.ba/}.

\bibitem{entel}
{Entel Bolivia}, 2020.
\newblock \url{https://www.entel.bo/}.

\bibitem{oui}
{IEEE OUI database}, 2020.
\newblock \url{http://standards-oui.ieee.org/oui.txt}.

\bibitem{starcat}
{Starcat Cable Network}, 2020.
\newblock \url{http://www.starcat.co.jp.e.lh.hp.transer.com/}.

\bibitem{imc16yarrp}
Robert Beverly.
\newblock {Yarrp'ing the Internet: Randomized High-Speed Active Topology
  Discovery}.
\newblock In {\em Proceedings of ACM Internet Measurement Conference (IMC)},
  November 2016.

\bibitem{imc18beholder}
Robert Beverly, Ramakrishnan Durairajan, David Plonka, and Justin~P. Rohrer.
\newblock {In the IP of the Beholder: Strategies for Active IPv6 Topology
  Discovery}.
\newblock In {\em Proceedings of ACM Internet Measurement Conference (IMC)},
  November 2018.

\bibitem{caida-routed48}
{CAIDA}.
\newblock {The CAIDA UCSD IPv6 Routed /48 Topology Dataset}, 2019.
\newblock
  \url{https://www.caida.org/data/active/ipv6\_routed\_48\_topology\_dataset.xml}.

\bibitem{rfc4443}
A.~Conta, S.~Deering, and M.~{Gupta (Ed.)}.
\newblock {Internet Control Message Protocol (ICMPv6) for the Internet Protocol
  Version 6 (IPv6) Specification}.
\newblock RFC 4443 (Internet Standard), March 2006.
\newblock Updated by RFC 4884.

\bibitem{rfc7721}
A.~Cooper, F.~Gont, and D.~Thaler.
\newblock {Security and Privacy Considerations for IPv6 Address Generation
  Mechanisms}.
\newblock RFC 7721 (Informational), March 2016.

\bibitem{durumeric2013zmap}
Zakir Durumeric, Eric Wustrow, and J~Alex Halderman.
\newblock Zmap: Fast internet-wide scanning and its security applications.
\newblock In {\em {22nd USENIX Security Symposium (USENIX Security 13)}}, pages
  605--620, 2013.

\bibitem{Gasser:2018:CEU:3278532.3278564}
Oliver Gasser, Quirin Scheitle, Pawel Foremski, Qasim Lone, Maciej
  Korczy\'{n}ski, Stephen~D. Strowes, Luuk Hendriks, and Georg Carle.
\newblock {Clusters in the Expanse: Understanding and Unbiasing IPv6 Hitlists}.
\newblock In {\em Proceedings of ACM Internet Measurement Conference (IMC)},
  2018.

\bibitem{anonymousemail}
AVM GmbH.
\newblock {EUI-64 Vulnerability Disclosure}.

\bibitem{rfc7707}
F.~Gont and T.~Chown.
\newblock {Network Reconnaissance in IPv6 Networks}.
\newblock RFC 7707 (Informational), March 2016.

\bibitem{rfc3177}
IAB and IESG.
\newblock {Recommendations on IPv6 Address Allocations to Sites}.
\newblock RFC 3177 (Informational), September 2001.

\bibitem{imc20facebook}
Frank Li and David Freeman.
\newblock {Towards A User-Level Understanding of IPv6 Behavior}.
\newblock In {\em Proceedings of ACM Internet Measurement Conference (IMC)},
  October 2020.

\bibitem{rfc4429}
N.~Moore.
\newblock {Optimistic Duplicate Address Detection (DAD) for IPv6}.
\newblock RFC 4429, April 2006.

\bibitem{rfc8415}
T.~Mrugalski, M.~Siodelski, B.~Volz, A.~Yourtchenko, M.~Richardson, S.~Jiang,
  T.~Lemon, and T.~Winters.
\newblock {Dynamic Host Configuration Protocol for IPv6 (DHCPv6)}.
\newblock RFC 8415 (Proposed Standard), November 2018.

\bibitem{rfc4941}
T.~Narten, R.~Draves, and S.~Krishnan.
\newblock {Privacy Extensions for Stateless Address Autoconfiguration in IPv6}.
\newblock RFC 4941 (Draft Standard), September 2007.

\bibitem{rfc6177}
T.~Narten, G.~Huston, and L.~Roberts.
\newblock {IPv6 Address Assignment to End Sites}.
\newblock RFC 6177 (Best Current Practice), March 2011.

\bibitem{atlas}
RIPE NCC.
\newblock {RIPE Atlas}, 2021.
\newblock \url{https://atlas.ripe.net/}.

\bibitem{akamaiblog}
Erik Nygren.
\newblock {At 21Tbps, Reaching New Levels of IPv6 Traffic}, 2020.
\newblock
  \url{https://blogs.akamai.com/2020/02/at-21-tbps-reaching-new-levels-of-ipv6-traffic.html}.

\bibitem{padmanabhan2020dynamips}
Ramakrishna Padmanabhan, John~P Rula, Philipp Richter, Stephen~D Strowes, and
  Alberto Dainotti.
\newblock {DynamIPs: Analyzing Address Assignment Practices in IPv4 and IPv6}.
\newblock In {\em Proceedings of the 16th International Conference on emerging
  Networking EXperiments and Technologies}, pages 55--70, 2020.

\bibitem{Plonka:2015:TSC:2815675.2815678}
David Plonka and Arthur Berger.
\newblock {Temporal and Spatial Classification of Active IPv6 Addresses}.
\newblock In {\em Proceedings of ACM Internet Measurement Conference (IMC)},
  2015.

\bibitem{rv}
{Routeviews}.
\newblock {University of Oregon Route Views Project}, 2020.
\newblock \url{http://www.routeviews.org/routeviews/}.

\bibitem{edgy}
Erik~C Rye and Robert Beverly.
\newblock {Discovering the IPv6 Network Periphery}.
\newblock In {\em International Conference on Passive and Active Network
  Measurement}, pages 3--18. Springer, 2020.

\bibitem{rfc4862}
S.~Thomson, T.~Narten, and T.~Jinmei.
\newblock {IPv6 Stateless Address Autoconfiguration}.
\newblock RFC 4862, September 2007.

\bibitem{kirstin}
Kirstin~E Thordarson.
\newblock {Analysis of EUI-64-Based Addressing and Associated Vulnerabilities}.
\newblock Master's thesis, Monterey, CA; Naval Postgraduate School, 2020.

\bibitem{zmap6}
tumi8.
\newblock {ZMapv6: Internet Scanner with IPv6 Capabilities}, 2021.
\newblock \url{https://github.com/tumi8/zmap}.

\end{thebibliography}

